Scheduling with Communication Delay in Near-Linear Time

We consider the problem of efficiently scheduling jobs with precedence constraints on a set of identical machines in the presence of a uniform communication delay. Such precedence-constrained jobs can be modeled as a directed acyclic graph, $G = (V, E)$. In this setting, if two precedence-constrained jobs $u$ and $v$, with $v$ dependent on $u$ ($u \prec v$), are scheduled on different machines, then $v$ must start at least $\rho$ time units after $u$ completes. The scheduling objective is to minimize makespan, i.e. the total time from when the first job starts to when the last job finishes. The focus of this paper is to provide an efficient approximation algorithm with near-linear running time. We build on the algorithm of Lepere and Rapine [STACS 2002] for this problem to give an $O\left(\frac{\ln \rho}{\ln \ln \rho} \right)$-approximation algorithm that runs in $\tilde{O}(|V| + |E|)$ time.

==> alg-ancestor-estimation.tex <==
\begin{algorithm}[hbtp]
\caption{Estimate Number of Ancestors}\label{alg:ancestor-estimation}
\SetAlgoLined
\KwResult{A small subgraph $H = (V', E')$.}
\textbf{Input: } A directed-acyclic graph $G = (V, E)$ and an accuracy parameter $\eps$.\\

Let $\NumberVertices{} \leftarrow |V|$.\\
Assign each node $v \in V$ a unique ID from $[n]$.\\
Intialize $V' \leftarrow \emptyset$.\\
Let $\info$ be an array of size $\NumberVertices{}$ (i.e. one entry per node). Initialize $\info[v] = \nul$ for all nodes $v \in V$.\\

\For{node $v \in V$ in topological order}{
  Compute $\pred(v)$ the set of immediate predecessors of $v$.\\
  Assign $\dist \leftarrow \nul$, which will be the estimator for $v$.\\
  Perform $\est$.insert$(\dist, v)$.\\
  \For{$u \in \pred(w)$}{
    Retrieve $\dist_u \leftarrow \info(u)$ the estimator for $u$.\\
    Perform $\est$.merge$(\dist, \dist_u)$.
  }
  Set $\info[v] = \dist$.\\
  \If{$\est$.estimateCardinality$(\dist) \le (1 + \eps)\CommunicationDelay{}$}{
    Add $v$ to $V'$.\\
  }
}
Create $H = (V', E')$ from $G$ by taking all edges between two vertices in $V'$.\\
Return $H$.\\
\end{algorithm}
